Automated Cardiovascular Record Retrieval by Multimodal Learning between Electrocardiogram and Clinical Report

Automated interpretation of electrocardiograms (ECG) has garnered significant attention with the advancements in machine learning methodologies. Despite the growing interest, most current studies focus solely on classification or regression tasks, which overlook a crucial aspect of clinical cardio-disease diagnosis: the diagnostic report generated by experienced human clinicians. In this paper, we introduce a novel approach to ECG interpretation, leveraging recent breakthroughs in Large Language Models (LLMs) and Vision-Transformer (ViT) models. Rather than treating ECG diagnosis as a classification or regression task, we propose an alternative method of automatically identifying the most similar clinical cases based on the input ECG data. Also, since interpreting ECG as images is more affordable and accessible, we process ECG as encoded images and adopt a vision-language learning paradigm to jointly learn vision-language alignment between encoded ECG images and ECG diagnosis reports. Encoding ECG into images can result in an efficient ECG retrieval system, which will be highly practical and useful in clinical applications. More importantly, our findings could serve as a crucial resource for providing diagnostic services in underdeveloped regions.

==> tables/ablation_encode.tex <==
\begin{tabular}{l|rrr|rrr|r}
\toprule 
\multirow{2}{*}{Encoding Method} & \multicolumn{3}{c}{Diagnosis Report Retrieval}  &\multicolumn{3}{c}{ECG Image Retrieval}  \\
& R@1 & R@5& R@10  &R@1 & R@5 & R@10  &RSUM \\
\midrule
MTF-only &1.42 &5.67 &10.72 &1.97 &6.07 &10.80 \\
GAF-only &2.69 &10.53 &17.04 &3.22 &11.01 &17.60 & \\
RP-only &5.27 &16.84 &25.68 &5.63 &17.20 &26.44 \\
\midrule
MTF+GAF &4.02 &14.03 &21.91 &4.10 &14.42 &21.91 \\
GAF+RP &6.30 &21.04 &30.36 &6.93 &20.69 &30.65 \\
PR+MTF &5.12 &17.26 &25.84 &4.96 &17.10 &26.56 \\
\midrule
All-Concat &1.58 &7.25 &12.77 &1.73 &7.33 &13.71 \\
All-Grid &7.88 &22.54 &32.23 &7.32 &21.91 &33.41\\
\bottomrule
\end{tabular}
